PromoPlot: Covering open-access fees by filling wasted space in corner plots

In an effort to reduce drain on grant funds and decrease unused space in publications, we have developed a Python package for inserting advertisements into the space left empty by corner plots. This novel technique can allow authors to reduce or eliminate publication charges for journals such as MNRAS and ApJ. In order to offset publication costs entirely, we recommend that authors include anywhere from 200-700 corner plots per paper, with the exact number depending on the journal used. Finally, we discuss other opportunities to generate ad revenue through publications.

==> old_intro.tex <==
\section{Introduction} \label{sec:intro}

The ascension of the open-access journal has been accompanied by increasing dependence on author publication fees. While this transition has strong merits in ensuring a wide dissemination of research, without subscription fees, publishers now rely on authors to cover the journal operating costs. As of last year, nearly 50\% of all papers are published in open-access or hybrid open-access journals where the author fronts the majority of the bill \citep{Brainard24}. In 2022, all journals published through the American Astronomical Society (AAS) switched to an open-access model. In 2024, the Monthly Notices of the Royal Astronomy Society (MNRAS) followed suit. While there are some journals, like the Open Journal of Astronomy, that are peer-reviewed, open-access, and do not have author publication costs, such journals are the clear exception. 

While open-access journals promote broader access to research and can increase visibility and impact, they have also served as effective sources of revenue for publishers. Between 2019 and 2023, \citet{Haustein24} found that the spending by authors on open-access fees nearly tripled, generating \$8.97 billion over the five-year period for a selection of six publishers.

In addition, by passing the costs to the authors, the ability to publish in high-impact journals becomes linked to the affluence of the author's country or institution. While some journals, including the AAS Journals \footnote{\url{https://journals.aas.org/support}} and MNRAS\footnote{\footnotesize\url{https://academic.oup.com/pages/purchasing/developing-countries-initiative/}}, offer waivers or discounts to scientists in low-income countries, it has been shown that these can still not be enough to incentive scientists to publish in open-access journals \citep{Momeni23}.


%As technology has advanced in recent years, the calling of scientists to distribute information to all has been easier and easier to fulfill. As popular emphasis on public availability of information has increased, the mantle has been taken up by the largest journals in Astronomy, as they shift to a new model. 

%In 2022, all journals published through the American Astronomical Society (AAS) switched to an open-access model. In 2024, the Monthly Notices of the Royal Astronomy Society (MNRAS) followed suit. Now, it seems that open access has become the standard, and subscription models for journals are the exception, not the norm. This transition carries with it a massive increase in the accessibility of information and research, and should be applauded. There is, however, an unfortunate side effect.

%The peer-review process is integral to science, but it is unfortunate that we must pay money to help others unravel the mysteries of the universe. Publishing papers to AAS could cost anywhere from \$1500-\$5000, money that could be used to fund even more research. 

Publication costs can range from \$1500-\$5000 per article, detracting from funds that can be used for conducting research, hiring students, and participating in conferences. It is unlikely that the open-access policies or author payment costs will change in the near future. We therefore are incentivized to identify opportunities to offset these costs. We can start by looking at sources of revenue generation used by other online media platforms that can be applied to scientific publications. The most common business model used online is advertisements. Entire services and website development packages have been built to seamlessly integrate advertisements on sites. In online media, ads are commonplace, appearing as banners or sidebars, pop-ups, or at bookends of online videos. 

%It is our belief that researchers need not suffer for their commitment to sharing knowledge with the scientific community and world at large. So we decided to search out a method to help offset these costs, by comparing with the other main form of information dispersal - websites. Personal websites share many similarities with journal articles: they cost money to host and allow authors to disseminate their information with a broader community. Websites typically offset operating fees through ad revenue, but not journal articles. Why is this? The answer is clear. Website development packages have prebuilt packages for adding advertisements to their pages but journal articles don't. So one must be created.

The most successful advertisements are carefully placed within the content so that they do not detract from the website or media. For example, using in-line advertisements that push the text around would make reading a paper just as unpleasant as trying to find the actual recipe on a recipe webpage.  Instead, our goal is to identify and fill space that is currently wasted and utilize that space to generate ad revenue.

%However, there is a concern. Websites implement advertisements in open space. Inserting in line advertisements that push the text around is a possible solution, but would make reading papers as unpleasant as trying to find the actual recipe on a recipe webpage

Here, we investigate how publication costs can be offset by taking advantage of space that is currently wasted in most manuscripts. The availability of open-source sampling codes, such as {\tt emcee} \citep{ForemanMackey13} and {\tt DYNESTY} \citep{Speagle20}, has made parameter estimation for complex, multimodal distributions commonplace in the literature. As a result, studies using these methods often present posteriors in the form of a ``triangle'' or ``corner'' plot. These are typically structured with histograms on the diagonal and the covariances for each parameter shown above or below the diagonal. These figures provide a straightforward way to view results of sampling methods, but they also render a substantial part of the page unusable, wasting valuable page costs. 

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/saving_space.pdf}
    \caption{With \packname{}, the amount of space wasted with corner plots can be reduced substantially. In this example, $\sim 25\%$ of the figure is now dedicated to advertising. This results a $\sim 57\%$ reduction in wasted space for this figure as well.}
    \label{fig:saving_space}
\end{figure*}

The prevalence of such figures is only increasing. As of April 1st, 2025, more than 1,700 papers cite the {\tt corner} package \citet{ForemanMackey16}, with more than 350 of these citations coming from 2024 alone. There have been approximately 400 papers citing {\tt corner} in both ApJ and MNRAS spanning a range of fields including exoplanets \citep{Jones24}, cosmology \citep{Turner24}, stars \citep{Rowan25}, and the interstellar medium \citep{Sun18}. In some cases, $\gtrsim 10$ corner plots are used in a single publication \citep[e.g.,][]{Calabrese2025}. 

We therefore propose to solve two problems -- page charges and wasted space in corner plots -- with a single solution by selling ad space in the upper half of corner plots. In Section \S\ref{sec:Implementation}, we present our Python package, \packname{}, and demonstrate how users can automatically include advertisements in their corner plots. In Section \S\ref{sec:profits}, we determine how much the use of ads in corner plots can reduce page charges. Finally, we describe the prospects for wide adoption of this practice in the field, and the possibilities for selling target ads. 


